CLASSO: a practical primal path-following algorithm for the constrained LASSO

We present CLASSO, a path-following method for the LASSO subject to general linear equality and inequality constraints. The local direction is obtained from a quadratic programme on an augmented active set, which determines both the coefficients that leave zero and the weakly active inequalities that remain binding. For a positive-definite Hessian and a nonempty feasible set, this programme has a unique primal minimiser, even when the binding constraint rows are dependent, and gives the local derivative of the solution path. The construction recovers the LASSO-modified LARS direction without constraints, and over the full cone gives the segment leaving the origin. We prove that the primal path is piecewise affine with finitely many kinks, without a constraint qualification or unique multipliers. A finite path does not imply a finite traversal: re-certifying at each kink can fail to terminate. CLASSO instead follows the minimum-norm certificate along a lexicographic rate; we prove that this rule reaches $\lambda=0$ in exact arithmetic within an explicit bound and traverses the whole path. These results are machine-checked in Lean~4, and the floating-point implementation agrees with an exact rational one on all $210$ small test problems. We assess the implementation on a $39$-case synthetic suite and six constrained versions of the diabetes benchmark. On the $31$ nontrivial synthetic cases with $n\ge p$, sampled relative objective differences from numerical reference solves are below $10^{-9}$ in magnitude; unnormalised endpoint differences reach $1.5\times10^{-7}$ in magnitude. For $n<p$, matched differences range from $-3.6\times10^{-7}$ to $2\times10^{-9}$ across five ridge strengths. Across the synthetic and diabetes benchmarks, checks of all $580$ recorded segments found no missed interior event and all checked KKT residuals within the stated tolerances.

==> cil-preamble.tex <==
% cil-preamble.tex -- shared, class-independent preamble for the
% Cambridge Inference CLASSO and CLARS papers.  Included by every
% wrapper (JCGS single-column and arXiv two-column).  Nothing here may
% depend on the document class: interact.cls already loads amsmath,
% amssymb, amsthm, booktabs, graphicx and rotating, so each of those is
% guarded below rather than loaded unconditionally.

\makeatletter

\@ifpackageloaded{graphicx}{}{\RequirePackage{graphicx}}
\@ifpackageloaded{amsmath}{}{\RequirePackage{amsmath}}
% newtxmath defines \Bbbk, which amssymb then refuses to redefine; the
% \let is needed only when we are the ones loading amssymb.
\@ifpackageloaded{amssymb}{}{\let\Bbbk\relax \RequirePackage{amssymb}}
\@ifpackageloaded{booktabs}{}{\RequirePackage{booktabs}}

\RequirePackage{bm}
\RequirePackage{subcaption}
\RequirePackage{algorithm}
\RequirePackage{algpseudocode}
\captionsetup{compatibility=false}

% mnras and interact each predefine \proof; amsthm must be allowed to
% install its own, but only if the class has not already loaded it.
\@ifpackageloaded{amsthm}{}{%
  \let\openbox\relax
  \let\proof\relax
  \let\endproof\relax
  \RequirePackage{amsthm}}

\makeatother

% mnras loads hyperref, which supplies \texorpdfstring; interact and
% article do not, and the body uses it in two section titles.
\providecommand{\texorpdfstring}[2]{#1}

\usepackage[noabbrev]{cleveref}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{remark}
\newtheorem{remark}{Remark}

% common maths expressions
\newcommand{\Z}{\ensuremath{\mathcal{Z}}}
\newcommand{\e}{\mathrm{e}}

% Several tables are wider than the measure in one or both layouts: the
% two-column reading version and the single-column submission version
% have very different line lengths. \CILFITWIDTH shrinks its argument
% only when it would otherwise overflow, so each layout scales exactly
% the tables it has to and leaves the rest untouched.
\newcommand{\CILFITWIDTH}[1]{%
  \resizebox{\ifdim\width>\linewidth \linewidth\else \width\fi}{!}{#1}}

% Float placement. LaTeX's defaults cap a top float at 0.7 of the text
% block, so a float taller than that cannot go at the top or bottom of a
% text page and is deferred to a page of its own, where it is centred and
% the remaining space left blank. Algorithm 1 is 0.8 of the block in the
% single-column layout and was being isolated for exactly that reason.
% Raising the caps lets a tall float head a text page; raising
% \floatpagefraction makes a float page the last resort it should be.
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.7}
\renewcommand{\textfraction}{0.07}
\renewcommand{\floatpagefraction}{0.85}
\renewcommand{\dbltopfraction}{0.9}
\renewcommand{\dblfloatpagefraction}{0.85}
\setcounter{topnumber}{3}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}
\setcounter{dbltopnumber}{3}

